Acyclic Strategy for Silent Self-Stabilization in Spanning Forests

In this paper, we formalize design patterns, commonly used in the self-stabilizing area, to obtain general statements regarding both correctness and time complexity guarantees. Precisely, we study a general class of algorithms designed for networks endowed with a sense of direction describing a spanning forest (e.g., a directed tree or a network where a directed spanning tree is available) whose characterization is a simple (i.e., quasi-syntactic) condition. We show that any algorithm of this class is (1) silent and self-stabilizing under the distributed unfair daemon, and (2) has a stabilization time which is polynomial in moves and asymptotically optimal in rounds. To illustrate the versatility of our method, we review several existing works where our results apply.

==> lower_round.tex <==
\subsection{Lower Bound in Rounds}

%% A REFAIRE

We now show that Algorithm $\mathcal{NOLP}$ has a stabilization time
is in $\Omega(n)$ rounds in any tree of height $H=1$.  This negative
result is mainly due to the fact that actions not locally mutually
exclusive. In the next section, we will propose a simple
transformation to obtain a stabilization time is in $O(H)$ rounds in
any case in the next subsection. We will also show that this latter
transformation does not affect the move complexity.

Our proof consists in exhibiting a possible execution that terminates
in $2n+2$ rounds assuming a central (unfair) daemon, that is, at each
step exactly one process executes an action. Notice that the central
daemon is a particular case of the distributed unfair daemon. Notice
also that in the execution we build below, except in a particular
case, all processes executes at least one action during each round and
the last process that executes in the round execute exactly one action
in the round.

%%%

\clearpage

\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
    \includegraphics[scale=0.25]{fig/omega_n_init}
 \caption{Configuration initial}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
     \includegraphics[scale=.25]{fig/omega_n_r2deb} 
     \caption{End of the first round}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\For{$i$}{0}{$n-1$}\Comment{Round 1}
\State $p_i$ executes $R(p_i)$
\EndFor
\end{algorithmic}

\begin{algorithmic}[1]
\For{$i$}{1}{$n-2$}\Comment{Rounds $i+1$ with $i\in\{1, ..., n-2\}$}
\State $p_i$ executes $S(p_i)$
\State $p_0$ executes $S(p_0)$
\For{$j$}{0}{$n-1$}
\State $p_j$ executes $R(p_j)$
\EndFor
\EndFor
\end{algorithmic}

\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
\includegraphics[scale=.25]{fig/omega_n_r2fin}
 \caption{End of the second round}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
    \includegraphics[scale=.25]{fig/omega_n_riplus1fin}
     \caption{Last configuration of Round $i+1$ with $i\in\{1, ..., n-2\}$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}



\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
      \includegraphics[scale=.25]{fig/new1}
 \caption{Last configuration of Round $n-1$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
      \includegraphics[scale=.25]{fig/new2}
     \caption{Last configuration of Round $n$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\State $p_{n-1}$ executes $S(p_{n-1})$\Comment{Round $n$}
\State $p_0$ executes $S(p_0)$
\end{algorithmic}

\bigskip

\begin{algorithmic}[1]
\State $p_0$ executes $R(p_0)$\Comment{Round $n+1$}
\end{algorithmic}

\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
      \includegraphics[scale=.25]{fig/new3}
 \caption{Last configuration of Round $n+1$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
    \includegraphics[scale=.25]{fig/omega_n_rnplus1fin}
     \caption{Last configuration of Round $n+2$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\For{$i$}{1}{$n-1$}\Comment{Round $n+2$}
\State $p_i$ executes $R(p_i)$
\EndFor
\State $p_0$ executes $C(p_0)$
\end{algorithmic}

\bigskip

\begin{algorithmic}[1]
\State $p_0$ executes $S(p_0)$\Comment{Round $n+3$}
\For{$i$}{1}{$n-1$}
\State $p_i$ executes $C(p_i)$
\EndFor
\end{algorithmic}


\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
     \includegraphics[scale=.25]{fig/omega_n_rnplus2fin}
 \caption{Last configuration of Round $n+3$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
     \includegraphics[scale=.25]{fig/omega_n_rnplus3fin}
     \caption{Last configuration of Round $n+4$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\For{$i$}{0}{$n-1$}\Comment{Round $n+4$}
\State $p_i$ executes $R(p_i)$
\EndFor
\end{algorithmic}

\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
     \includegraphics[scale=.25]{fig/omega_n_rnplus3plus1fin}
 \caption{Last configuration of Round $n+5$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
       \includegraphics[scale=.25]{fig/omega_n_rnplus3plusifin}
     \caption{Last configuration of Round $n+4+i$ with $i \in \{1, ...,  n-2\}$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\For{$i$}{1}{$n-2$}\Comment{Round  $n+4+i$ with $i \in \{1, ...,  n-2\}$}
\State $p_i$ executes $S(p_i)$
\State $p_0$ executes $S(p_0)$
\For{$j$}{0}{$n-1$}
\State $p_j$ executes $R(p_j)$
\EndFor
\EndFor
\end{algorithmic}


\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
     \includegraphics[scale=.25]{fig/new4}
 \caption{Last configuration of Round $2n+2$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
      \includegraphics[scale=.25]{fig/new5}
     \caption{}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}

\begin{algorithmic}[1]
\State $p_{n-1}$ executes $S(p_{n-1})$\Comment{Round  $2n+3$}
\end{algorithmic}

\bigskip

\begin{algorithmic}[1]
\State $p_{0}$ executes $S(p_{0})$\Comment{Round  $2n+4$}
\end{algorithmic}

\begin{figure} [H]
\begin{minipage}{.48\linewidth}
  \begin{center}
      \includegraphics[scale=.25]{fig/new6}
 \caption{Last configuration of Round $2n+4$}
 \end{center}
 \end{minipage}
\hfill
\begin{minipage}{.48\linewidth}
  \begin{center}
  \includegraphics[scale=.25]{fig/new7}
     \caption{Last configuration of Round $2n+5$}
 \end{center}
 \end{minipage}
%\hfill
\end{figure}


\begin{algorithmic}[1]
\State $p_{0}$ executes $R(p_{0})$\Comment{Round  $2n+5$}
\end{algorithmic}

\bigskip

\begin{algorithmic}[1]
\For{$i$}{1}{$n-1$}\Comment{Round  $2n+6$}
\State $p_i$ executes $R(p_i)$
\EndFor
\end{algorithmic}

\begin{figure} [H]
  \begin{center}
      \includegraphics[scale=.25]{fig/omega_n_rnplus3plusnmoinsunfin}
     \caption{Last configuration of Round $2n+6$: terminal configuration}
 \end{center}
%\hfill
\end{figure}

% \clearpage

% Starting from the configuration given in Figure~\ref{init}. The first
% round consists in correcting the variables $Res$ of all processes. The
% root executes first so that $r.Res$ takes value $n$. Then, $n$ is
% propagated into all other variables $Res$.  Hence, the daemon executes
% the following algorithm to achieve Round 1.



% Hence, the last configuration of the first round ({\em i.e}, the first
% configuration of the second round) is the one given in Figure
% \ref{deb2}. Starting from that configuration, the $n-1$ next rounds consists in correcting the value of the variable $Sub$ of some leaf process, then updating $r.Sub$, and finally propagating $r.Sub$ in all $Res$ variables as in Round 1. 
% Hence,the daemon executes
% the following algorithm to achieve Rounds $i+1$, for all $i \in \{1, ...,  n-1\}$.



% The first of this round (that is, Round 2) leads to the configuration given in 
%  Figure
% \ref{fin2}. 



% Each round $i+1$, with $i \in \{1, ...,  n-1\}$ terminates in the
% configuration given in Figure \ref{fin_i}. Hence, the last
% configuration of Round $n$ is the one given in Figure \ref{fin_n}.




==> toy.tex <==
\section{Toy Example}

In this section, we propose an example of algorithm, called Algorithm
$\mathcal{NOLP}$, whose termination and complexity can be simply
deduced from our general results.
%
This algorithm assumes that the network $T = (V,E)$ is a tree ({\em
  i.e.}, an undirected connected acyclic graph) with a sense of
direction (given by variables $parent$ and $children$) which defines a
spanning in-tree rooted at process $r$ (the unique root, {\em i.e.},
the unique process satisfying $r.parent = \perp$).
%
The aim of $\mathcal{NOLP}$ (stands for {\em Number of Odd Level
  Processes}) is to compute the number of processes in the tree whose
level is odd. The algorithm consists of one bottom-up and two top-down
families of actions.  The first top-down family consists in
computing a 2-coloring of the tree such that a node takes color 1 if
its level in the tree is odd, 0 otherwise. Hence, we introduce a
variable $p.Clr \in \{0,1\}$, for every node $p$, and the top-down
family, called $C$: $$C(r)\ ::\ r.Clr \neq 0\ \to\ r.Clr
\gets 0$$
%
For every node $p \neq r$ 
%
$$C(p)\ ::\ p.Clr \neq (p.parent.Clr + 1) \bmod 2 \ \to\
p.Clr \gets (p.parent.Clr + 1) \bmod 2$$

Remark that $C$ is top-down and correct-alone.  The second family of actions
is bottom-up and aims at computing the number of odd-level processes
in the subtree $T(p)$, for every node $p$. The guideline to implement
this family is to assume that all $p.Clr$ are correctly
evaluated. Hence, we can introduce a variable $p.Sub \in \mathds N$,
for every node $p$, and the bottom-up family of actions, called $S$:

For every node $p$ 
$$
S(p)\ ::\ 
p.Sub \neq (\sum_{q \in p.children} q.Sub) + p.Clr\
\to\ p.Sub \gets (\sum_{q \in p.children} q.Sub) + p.Clr
$$

Remark that $S$ is bottom-up and correct-alone. Assuming the
$p.Sub$ is correctly computed at each node $p$, the last family
consists in propagating the result, $r.Sub$, in a top-down
manner. Hence, we introduce a variable $p.Res \in \mathds N$, for
every node $p$, and the top-down family, called $R$:

$$R(r)\ ::\ r.Res \neq r.Sub\ \to\ r.Res \gets r.Sub$$
%
For every node $p \neq r$ 
%
$$R(p)\ ::\ p.Res \neq p.parent.Res\ \to\ p.Res \gets p.parent.Res$$

Remark that $R$ is top-down and correct-alone. Then the graph of actions' causality of $\mathcal{NOLP}$ is

$$C \to S \to R$$
So, we can apply Corollary~\ref{coro:moves} (we have $\DeltamGC=1$,
$\HGC=2$ and $k=3$), every execution of $\mathcal{NOLP}$ contains at
most $3(2+\DeltaG)^2.n^4$ moves and, as a direct consequence, every
execution of $\mathcal{NOLP}$ terminates under the distributed unfair
daemon. Notice also that is every terminal configuration, every node
$p$ satisfies the following properties:
\begin{enumerate}
\item $p.Clr = 0$ {\bf if} $p = r$, $p.Clr = (p.parent.Clr + 1) \bmod 2$
  {\bf otherwise},
\item $p.Sub = p.Clr+\sum_{q \in p.children} q.Sub$,
\item $p.Res = p.Sub$ {\bf if} $p = r$, $p.Res = p.parent.Res$
  {\bf otherwise}.
\end{enumerate}
Let $P_{\mathcal{NOLP}} \equiv \forall p \in V, p.Res = |\{q \in V, L(q)\bmod
2 = 1 \}|$, where $L(q)$ is the level of $q$ in
$T$.

By induction, we can deduce that $P_{\mathcal{NOLP}}$ in any terminal
configuration of $\mathcal{NOLP}$. Hence, by Theorem
\ref{theo:silentself}, follows.
\begin{theorem}
  $\mathcal{A}$ is silent and self-stabili\-zing
  for~$P_{\mathcal{NOLP}}$ in $T$ under a distributed unfair daemon,
  and its stabilization time is at most $3(2+\DeltaG)^2.n^4$ moves.
\end{theorem}

Using Lemma~\ref{lem:moves} directly, the move complexity of
$\mathcal{NOLP}$ can be further refined. Let $e$ be any execution of
$\mathcal{NOLP}$ and $\HG$ be the height of $T$. First, note that,
$maxO(C) = maxO(S) = maxO(R) = 0$, by
Remark~\ref{rem:maxO}.

\begin{enumerate}
\item Since $C$ is top-down, $|Z(p,C)| \leq \HG+1$, for
  every node $p$. Moreover, the height of $C$ is 0 in the graph
  of actions' causality. Hence, by Lemma~\ref{lem:moves}, we have
  $\#m(e,C,p) \leq \HG+1$, for all processes $p$. Hence, $e$
  contains at most $(\HG+1).n$ moves of $C$.
\item Since $S$ is bottom-up, $|Z(p,C)| \leq n$, for
  every node $p$. Moreover, the height of $S$ is 1 in the graph
  of actions' causality. Hence, by Lemma~\ref{lem:moves}, we
  have $\#m(e,S,p) \leq 2.n^2$, for all processes $p$.
Hence, $e$
  contains at most $2.n^3$ moves of $S$.
\item Since $R$ is top-down, $|Z(p,R)| \leq
  \HG+1$, for every node $p$. Moreover, the height of $R$
  is 2 in the graph of actions' causality. Hence, by
  Lemma~\ref{lem:moves}, we have $\#m(e,R,p) \leq
  4.n^2.(\HG+1)$, for all processes $p$. Hence, $e$ contains at most
  $4.n^3.(\HG+1)$ moves of $R$.
\end{enumerate}
Hence, overall, we have

\begin{theorem}
  The stabilization time of $\mathcal{NOLP}$ is at most
  $(\HG+1).n+2.n^3+4.(\HG+1).n^3$ moves, {\em i.e.}, $O(\HG.n^3)$
  moves.
\end{theorem}



